NSF-MAP: Neurosymbolic Multimodal Fusion for Robust and Interpretable Anomaly Prediction in Assembly Pipelines

In modern assembly pipelines, identifying anomalies is crucial in ensuring product quality and operational efficiency. Conventional single-modality methods fail to capture the intricate relationships required for precise anomaly prediction in complex predictive environments with abundant data and multiple modalities. This paper proposes a neurosymbolic AI and fusion-based approach for multimodal anomaly prediction in assembly pipelines. We introduce a time series and image-based fusion model that leverages decision-level fusion techniques. Our research builds upon three primary novel approaches in multimodal learning: time series and image-based decision-level fusion modeling, transfer learning for fusion, and knowledge-infused learning. We evaluate the novel method using our derived and publicly available multimodal dataset and conduct comprehensive ablation studies to assess the impact of our preprocessing techniques and fusion model compared to traditional baselines. The results demonstrate that a neurosymbolic AI-based fusion approach that uses transfer learning can effectively harness the complementary strengths of time series and image data, offering a robust and interpretable approach for anomaly prediction in assembly pipelines with enhanced performance. \noindent The datasets, codes to reproduce the results, supplementary materials, and demo are available at https://github.com/ChathurangiShyalika/NSF-MAP.

==> table.tex <==
\begin{table*}
\scriptsize
\begin{minipage}{0.6\textwidth}
\caption{Experimental Results of PredictX and Ablation Studies (mean(\%) ± std(\%)). Support: Number of samples used. Bold indicates the best performance.D: model used only for Detection.}
\label{tab:results}
\begin{tabular}{c|c|c|c|c|c|c|c|c} 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Training/}\\\textbf{Testing}\\\textbf{Split}\end{tabular} & \multicolumn{4}{c|}{\textbf{80 \% 20\%}}                                                                                                                                                                                                                                                                                                                                      & \multicolumn{4}{c}{\textbf{60 \% 40\%}}                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ 
\hline
\textbf{Model}                                                                               & \begin{tabular}[c]{@{}c@{}}\textbf{Weighted }\\\textbf{Avg.}\\\textbf{Precision}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Weighted }\\\textbf{Avg.}\\\textbf{Recall}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Weighted }\\\textbf{Avg.}\\\textbf{F1-Score}\end{tabular} & \textbf{Accuracy}                                                                 & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Weighted}}\\\textbf{\textbf{Avg.}}\\\textbf{\textbf{Precision}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Weighted}}\\\textbf{\textbf{Avg.}}\\\textbf{\textbf{Recall}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{Weighted}}\\\textbf{\textbf{Avg.}}\\\textbf{\textbf{F1-Score}}\end{tabular} & \textbf{\textbf{Accuracy}}                                                                                    \\ 
\hline
B1                                                                                           & \begin{tabular}[c]{@{}c@{}}74.00±\\1.00\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}63.00±\\1.00\%\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}}61.00±\\1.00\%\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}63.00±\\1.00\%\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}64.00±\\1.00\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}53.00±\\1.00\%\end{tabular}                                                               & \begin{tabular}[c]{@{}c@{}}51.00±\\1.00\%\end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}53.00±\\1.00\%\end{tabular}                                                        \\ 
\hline
B2: *D                                                                                       & \begin{tabular}[c]{@{}c@{}}97.00±\\1.05\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}97.00±\\0.5\%\end{tabular}                                      & \begin{tabular}[c]{@{}c@{}}97.00±\\1.00\%\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}97.00±\\1.00\%\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}87.00±\\1.05\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}87.00±\\0.5\%\end{tabular}                                                                & \begin{tabular}[c]{@{}c@{}}87.00±\\1.00\%\end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}87.00±\\1.00\%\end{tabular}                                                        \\ 
\hline
DLF (P1)                                                                                     & \begin{tabular}[c]{@{}c@{}}76.05±\\2.00\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}72.00±\\1.70\%\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}}72.03±\\2.05\%\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}72.00±\\2.00\%\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}66.05±\\2.00\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}62.00±\\1.70\%\end{tabular}                                                               & \begin{tabular}[c]{@{}c@{}}64.00±\\0.5\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}64.00±\\0.05\%\end{tabular}                                                        \\ 
\hline
\begin{tabular}[c]{@{}c@{}}DLF (TS+\\zero tensor\\image)\end{tabular}                        & \begin{tabular}[c]{@{}c@{}}80.00±\\1.00\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}64.00±\\0.5\%\end{tabular}                                      & \begin{tabular}[c]{@{}c@{}}64.00±\\0.5\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}64.00±\\0.05\%\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}70.00±\\1.00\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}60.00±\\0.5\%\end{tabular}                                                                & \begin{tabular}[c]{@{}c@{}}58.00±\\0.5\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}58.00±\\0.05\%\end{tabular}                                                        \\ 
\hline
\begin{tabular}[c]{@{}c@{}}DLF+TL \\(P2)\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}91.00±\\0.05\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}88.02±\\0.05\%\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}}89.00±\\0.05\%\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}88.00±\\0.05\%\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}81.00±\\0.05\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}78.02±\\0.05\%\end{tabular}                                                               & \begin{tabular}[c]{@{}c@{}}79.00±\\0.05\%\end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}78.00±\\0.05\%\end{tabular}                                                        \\ 
\hline
DLF+KIL                                                                                      & \begin{tabular}[c]{@{}c@{}}93.00±\\1.00\%\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}90.00±\\0.05\%\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}}91.00±\\0.05\%\end{tabular}                                       & \begin{tabular}[c]{@{}c@{}}90.00±\\0.05\%\end{tabular}                            & \begin{tabular}[c]{@{}c@{}}83.00±\\1.00\%\end{tabular}                                                                  & \begin{tabular}[c]{@{}c@{}}80.00±\\0.05\%\end{tabular}                                                               & \begin{tabular}[c]{@{}c@{}}81.00±\\0.05\%\end{tabular}                                                                 & \begin{tabular}[c]{@{}c@{}}80.00±\\0.05\%\end{tabular}                                                        \\ 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{DLF+TL+}\\\textbf{KIL(P3)}\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}\textbf{94.00±}\\\textbf{1.00\%}\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}\textbf{93.00±}\\\textbf{0.75\%}\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}\textbf{93\textbf{.00}±}\\\textbf{0.05\%}\end{tabular}            & \begin{tabular}[c]{@{}c@{}}\textbf{93\textbf{.00}±}\\\textbf{1.00\%}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{84.00±}}\\\textbf{\textbf{1.00\%}}\end{tabular}                              & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{83.00±}}\\\textbf{\textbf{0.75\%}}\end{tabular}                           & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{83\textbf{\textbf{.00}}±}}\\\textbf{\textbf{0.05\%}}\end{tabular}           & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{83\textbf{\textbf{.00}}±}}\\\textbf{\textbf{1.00\%}}\end{tabular}  \\
\hline
\end{tabular}
\end{minipage}
    \hfill
\begin{minipage}{0.27\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/rocket.pdf}
        \captionof{figure}{A Rocket Assembled by the Future Factories Lab. Any missing part is considered an anomaly: for example, the absence of Rocket body 1 is labeled as "NoBody1," while the absence of both Rocket body 1 and body 2 is labeled as "NoBody2, NoBody1."}
        \label{fig:rocket}
    \end{minipage}
    
\end{table*}
